Understanding the Humans Behind Online Misinformation: An Observational Study Through the Lens of the COVID-19 Pandemic

The proliferation of online misinformation has emerged as one of the biggest threats to society. Considerable efforts have focused on building misinformation detection models, still the perils of misinformation remain abound. Mitigating online misinformation and its ramifications requires a holistic approach that encompasses not only an understanding of its intricate landscape in relation to the complex issue and topic-rich information ecosystem online, but also the psychological drivers of individuals behind it. Adopting a time series analytic technique and robust causal inference-based design, we conduct a large-scale observational study analyzing over 32 million COVID-19 tweets and 16 million historical timeline tweets. We focus on understanding the behavior and psychology of users disseminating misinformation during COVID-19 and its relationship with the historical inclinations towards sharing misinformation on Non-COVID domains before the pandemic. Our analysis underscores the intricacies inherent to cross-domain misinformation, and highlights that users' historical inclination toward sharing misinformation is positively associated with their present behavior pertaining to misinformation sharing on emergent topics and beyond. This work may serve as a valuable foundation for designing user-centric inoculation strategies and ecologically-grounded agile interventions for effectively tackling online misinformation.

==> sections/ethics_checklist.tex <==
\subsection{Paper Checklist} % to be included in your paper}

%\mdc{What is ``paper checklist''? That's the language they want?}
%\mohit{Yes this is the exact subheading they used in the overleaf document}

\begin{enumerate}

\item For most authors...
\begin{enumerate}
    \item  Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
    \answerYes{Yes. The goal of this paper is to understand the behavior of the users who spread misinformation around COVID-19 and how it relates to their misinformation sharing activities historically and across various topics. We understand that user-centric research like ours, need to be careful about how the research is conducted, as unintended harms may result from specific forms of user profiling, categorization, labeling, or behavioral tracking. Therefore, we have adopted the best practices in social media research and  
    only presented aggregated results on users based on their misinformation-spreading tendency. Further, working deidentified data, we have only used the post content on an aggregated basis throughout our analysis and did not use any meta-data associated with the user (e.g., gender or racial inference, location, social status etc.) that could be used for unfair user profiling, exacerbating the socio-economic divide, or violating privacy norms.}
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Yes, please refer to the Abstract and Section~\ref{sec:introduction} in the main paper, that clearly outlines our major contributions that follow from our work.}
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
    \answerYes{Yes, we have clarified and justified the appropriateness of using the specific methodology at the start of each RQ section. Please refer to Sections~\ref{sec:rq1}, ~\ref{sec:rq2}, and ~\ref{sec:rq3} for further details, and Figure~\ref{fig:data_pipeline} to understand the overall data collection and user classification approach.}
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
    \answerYes{Yes, we have provided the details about statistics such as total number of posts, total number of \misinfo/\nonmisinfo~posts and the distribution of users among the each category in Table~\ref{tab:data_stats} and Section~\ref{sec:data_collection_clasification}.}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, please refer to Section~\ref{sec:conclusion_limitation} of the main paper.}
  \item Did you discuss any potential negative societal impacts of your work?
      \answerYes{Yes, we have discussed the potential negative societal impacts of our work in Section~\ref{sec:discussion} under ``Practical Strategies and Solutions'' $\rightarrow$ ``Empathetic solutions''. To elaborate, our study is centered on the examination of user behavior, with a specific focus on investigating the correlation between users' historical tendencies in disseminating misinformation and their present behavior in this regard. Consequently, there exists a conceivable risk of misusing the insights from our work if users on social media platforms are subject to biased tracking or inoculation-based interventions solely based on their historical behaviors, particularly regarding the anticipation of future misinformation sharing. The act of deplatforming users predicated on such anticipations has the potential to \textbf{limit users' freedom of expression}. Moreover, preemptively moderating users assuming they might share misinformation in the future may have chilling effects on speech, negatively impacting the online ``public sphere'' that may social media platforms aspire to be. Preemptive user moderation can also \textbf{disempower individuals} from developing critical thinking skills and media literacy. As we emphasize in Section~\ref{sec:discussion} under ``Practical Strategies and Solutions'' $\rightarrow$ ``Agile strategies'', it is important that our findings inspire approaches to promote media literacy and critical thinking, alongside inoculation efforts. Next, we note that as preemptive strategies become more sophisticated, those spreading misinformation may also \textbf{adapt and find new ways to evade detection} or counter the interventional efforts. Thus our findings should be interpreted and used in a way that adopts a collaborative approach to countering online misinformation, rather than villifying or victimizing certain individuals. We have discussed this under ``Practical Strategies and Solutions'' $\rightarrow$ ``Agile strategies'' of Section~\ref{sec:discussion}. Finally, we cannot ignore potential counterproductive reactions resulting from following some of the practical strategies and solutions we propose in this paper. Some research and media advocates suggest that directly confronting people with information that contradicts their beliefs can lead to a ``\textbf{backfire effect}," where they become more entrenched in their views. Potential preemptive interventions or inoculation efforts targeted at social media users thus need to be carefully designed to avoid unintentionally reinforcing misinformation.}
      \item Did you discuss any potential misuse of your work?
    \answerYes{Yes, we have discussed the potential misuse of our work in Section~\ref{sec:discussion} under ``Practical Strategies and Solutions'' $\rightarrow$ ``Empathetic solutions''. Building on these ideas, we note that user tracking by bad actors may result in \textbf{selective enforcement}. Deciding what counts as misinformation and what does not can be subjective, and there is a risk that inoculation efforts based on users' historical misinformation-sharing behaviors could be misused selectively to target certain viewpoints or political ideologies, leading to accusations of bias and censorship. }
    \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
    \answerYes{Yes, we have discussed the ethical aspects related to data curation, anonymization and responsible release in the \textbf{Broader perspective, ethics and competing interests} subsection under Section~\ref{sec:introduction}, as well as under ``Practical Strategies and Solutions'' in Section~\ref{sec:discussion}. Additionally, we have provided the code for the various misinformation classifiers through a link to an anonymous GitHub repository in the paper (which will be deanonymized upon acceptance). We plan to release our curated dataset with the Tweet IDs on a public GitHub repository, abiding by Twitter's policies.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes, our work follows the ethics guidelines.}
\end{enumerate}

\item Additionally, if your study involves hypotheses testing...
\begin{enumerate}
  \item Did you clearly state the assumptions underlying all theoretical results?
    \answerNA{NA}
  \item Have you provided justifications for all theoretical results?
    \answerNA{NA}
  \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
    \answerNA{NA}
  \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
    \answerNA{NA}
  \item Did you address potential biases or limitations in your theoretical framework?
    \answerNA{NA}
  \item Have you related your theoretical results to the existing literature in social science?
    \answerNA{NA}
  \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
    \answerNA{NA}
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{NA}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{NA}
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Yes, we have included the code along with the datasets used for fine-tuning the classifiers in an anonymous Github repository and provided a link to it in the main paper. Link to the anonymous GitHub repository is: \textit{https://tinyurl.com/icwsm24sub}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Yes, we have specified details about the model structure and hyperparameters in the main paper in Section~\ref{sec:data_collection_clasification}.}
     \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Yes, we have reported the standard error for each classifier across all the reported metrics based on 1) a 10-fold cross-validation and 2) with a random seed 42. These numbers can be found in  Table~\ref{tab:classifier_performance}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Yes, we fine-tuned each classifier using a single GPU on Google Colaboratory. None of the classifiers we built and evaluated took more than 12 hours to fine-tune.}
     \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made? 
    \answerYes{Yes, we used Accuracy, Precision, Recall, and F-1 score to show that the classifiers performed well in the misinformation classification task. Details can be found in Table~\ref{tab:classifier_performance}.}
     \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
     \answerYes{Yes, we discuss the cost of misclassification and the robustness of our study design here, as classification is not the core or sole focus of this paper. Our work employs an automated data labeling methodology using trained machine learning classifiers. While, these classifiers perform well over the used metrics (Accuracy, Precision etc; ref. Table~\ref{tab:classifier_performance}), we acknowledge that inaccuracies in the classification process may still arise, particularly for challenging cases. Our study tries to address this potential issue by conducting our analysis at the user level, as opposed to the post level, while also applying empirically-driven appropriate thresholds pertaining to the number and ratio of misinformative tweets (as mentioned in Section~\ref{sec:data_collection_clasification}). Through the implementation of these thresholds for user-level classification, we ensure the robustness of our analytical approach against misclassifications produced by the classifiers. Although our study's design has been structured to establish a high degree of robustness, it is important to acknowledge the possibility of occasional misclassifications at the user level. Nevertheless, it is noteworthy that the overarching findings of this study are expected to exhibit consistency and similarity when examined at an aggregated level.}
  
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Yes, we have cited the works/authors of the datasets we have used in our work.}
  \item Did you mention the license of the assets?
    \answerYes{Yes, we have mentioned that the datasets used for fine-tuning each classifier were publicly available in Section~\ref{sec:data_collection_clasification}.}
  \item Did you include any new assets in the supplemental material or as a URL?
    \answerYes{Yes, we have included a link to an anonymous Github repository in the main paper. The repository contains the following items: 
    \begin{itemize}
        \item Code used for the COVID-19, \politics~and \climate~misinformation classifiers.
        \item Datasets used for fine-tuning each classifier.
        \item Keyword list used for filtering out \politics~and \climate~tweets.
    \end{itemize}
    Please note that, we aim to release the Tweet IDs used for this study on the acceptance of this work, following adequate guidelines for data-sharing from Twitter/X.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{Yes, from our description in Section~\ref{sec:introduction} under ``Broader perspective, ethics and competing interests'' it follows that informed consent was not required in this work due to the publicly accessible nature of the Twitter posts, a focus on historical user posts and activities only (an observational study design), and the absence of any interaction between the researchers and the users. Due to these reasons, our research did not constitute human subjects research, per our Institutional Review Board (IRB), and thus seeking user consent was not applicable.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
     \answerYes{Yes, we worked with deidentified data only and all analyses on raw data was conducted using automated machine learning and natural language analysis tools, without needing to access any personally identifiable information (PII). Moreover, our curated dataset meant for public access will only have the Tweet IDs without any link to the PII of associated users or any potential offensive content. We have discussed this in detail in the \textbf{Broader perspective, ethics and competing interests} subsection of Section~\ref{sec:introduction}.}
\item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR (see \citet{fair})?
\answerYes{Yes, our curated dataset follows the FAIR principles and the Twitter data-sharing policy. As also mentioned before, we plan to release the Tweet IDs of the posts we have used in our work, without linking them to any PII directly. The Tweet IDs will be publicly available through our Github repository. These Tweet IDs can be used to retrieve the entire information pertaining to the Tweet (including the metadata) using the Twitter API or other data collection approaches crafted or advocated by X.}
\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset (see \citet{gebru2021datasheets})? 
\answerYes{Yes, we plan to release a datasheet for the curated dataset containing the Tweet IDs on our Github repository upon the acceptance of this paper. The datasheet will include the code for hydrating the Tweet IDs along with a reference to the keyword lists used for filtering the \politics~and \climate~data. During the course of preparation of this datasheet, we will abide by all relevant and up-to-date data-sharing guidelines of Twitter/X.}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots?
    \answerNA{NA, as this study did not constitute human subjects research (see our response to item 5(d) above).}
  \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
    \answerNA{NA, as this study did not constitute human subjects research, thus not required IRB approval (see our response to item 5(d) above).}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{NA, as this study did not constitute human subjects research (see our response to item 5(d) above).}
   \item Did you discuss how data is stored, shared, and deidentified?
   \answerNA{NA, this study did not constitute human subjects research and there was no interaction of the researchers with the social media users whose data was analyzed (see our response to item 5(d) above).} %\mohit{Not sure about this}
\end{enumerate}

\end{enumerate}





==> sections/related_work_cscw_extended.tex <==

%cite similar dataset and analysis and ML classifier papers. Then write a line or two about their major contributions


\subsection{Detection and analysis of online misinformation}

\subsubsection{Single Domain Misinformation}

The detection and trend analysis of misinformation across diverse topics on social media has garnered substantial scholarly attention in recent times. %Therefore, different aspects related to COVID-19 misinformation on online platforms have been studied extensively.
Focusing on COVID-19 misinformation, studies have focused on various topics, such as creating datasets, and social media content analysis. \citet{cui2020coaid} introduced the CoAID dataset that included over 4,200 news articles, 296,000 related user engagements, and 926 social platform posts about COVID-19. The authors further conducted a prescriptive analysis of misinformative hashtags and claims related to COVID-19. In another study, \citet{micallef2020role} curated a dataset of false claims and statements for counter-misinformation on fake cures and 5G conspiracy theories related to COVID-19. The study further revealed that non-fact-checker accounts generated 96\% of tweets refuting COVID-19-related misinformation. Furthermore, professional fact-checks were lower in tweet volume and received a significantly lower number of retweets than misinformative tweets. 


In a later study, \citet{10.1145/3465336.3475111} presented the CoronaBias dataset containing over 440,000 tweets focusing on Islamophobia during COVID-19. The authors additionally employed a classifier to identify Islamophobic content in the initial stages of the COVID-19 pandemic, revealing the emergence of an escalating anti-Muslim narrative propagated by a specific subset of users. On a related tangent, content analysis on different social media platforms has attracted a large number of studies. In one of the early studies,~\citet{kouzycovid} analyzed the correlation between different accounts (individual, public figures) and hashtags with the rate of misinformation spread. The authors found misinformation prevalence notably elevated among accounts affiliated with informal individuals or groups. Furthermore, tweets originating from unverified Twitter accounts exhibited a higher incidence of misinformation. \citet{li2022youtube} on the other hand, analyzed Youtube videos and found that over one-quarter of the most viewed YouTube videos on COVID-19 contained misleading information during March 2020. The study further revealed that 11\% of YouTube’s most viewed
videos on COVID-19 vaccines contradicted information from the WHO or CDC.

Recently, political misinformation and fake news has drawn attention from researchers, especially dissemination of misinformation during elections has been studied extensively.~\citet{article2016politicsfakenews} found that 25\% of tweets sharing news links during the 2016 US presidential elections promoted fake news. Further, the authors observed that users disseminating fake and highly biased news, albeit in smaller in number, not only exhibited heightened activity levels on average, but were also observed to be more extensively connected, through retweets, to a greater number of users when compared to individuals within traditional news networks. A few studies have also focused on creating datasets and classifiers for detecting political misinformation. In another study,~\citet{allcott2017social} highlighted the importance of social media in the dissemination of political news and focused on offering a theoretical and empirical background to political misinformation. The authors underscored the significance of comprehending the economic dynamics underlying the generation and dissemination of misinformation as a strategic approach for addressing the issue.~\citet{wang2017liar} presented the LIAR dataset comprising 12.8K manually labeled short statements collected from PolitiFact.com. Each statement was provided a single label from one of the six categories based on the degree of truthfulness-- `pants-fire,' `false,' `barely true,' `half-true,' `mostly-true,' and `true'. The authors also proposed a hybrid CNN-based deep learning architecture using text and meta-data for misinformation detection. Another noted study proposed FakeNewsNet, a repository containing 1,056 news articles and tweets related to real and fake news verified via PolitiFact and Gossip Cop~\cite{shu2020fakenewsnet}. In contrast, misinformation detection pertaining \climate~is relatively under-studied. Only a few studies include datasets focusing on climate change misinformation,~\citet{bhatia2020right} created a dataset comprising 1,168 articles focusing on climate change-related misinformation collected from 15 different CCCM organizations and reputed news sources. In a later study, \citet{diggelmann2021climatefever} proposed CLIMATE-FEVER dataset comprising 1,535 real-world claims on climate change along with relevant evident sentences labeled as one of `supporting,' `refuting' or `not enough information'.

Majority of the prior research has examined COVID-19, \politics, and \climate~misinformation separately, but this compartmentalized approach does not mirror real-world complexity, where users often encounter misinformation covering multiple topics. In contrast, our study delves into cross-domain misinformation, revealing the intricate interplay among various topics during the pandemic.


\subsubsection{Cross-Domain Misinformation}

While the past literature on detection and analysis of online misinformation has primarily focused on single domain such as COVID-19, there have been a handful of past works focusing on cross-domain misinformation detection. ~\citet{silva2021embracing} proposed a multimodal
fake news detection framework that learns domain-specific
and cross-domain information from news from three domains -- politics, entertainment industry and COVID-19. The proposed framework outperformed state-of-the-art fake news
detection models by 7.55\% in F1-score. In a later study,~\citet{10.1145/3485447.3512258} proposed a reinforcement learning-based model called REinforced Adaptive Learning Fake News Detection (REAL-FND) using domain-independent features to distinguish between fake and legitimate news. However, the domains explored in the paper were related to politics and the entertainment industry. However, as shown by~\citet{rastogi2021adaptive}, classifiers trained on specific single-domain data outperform classifiers trained on cross-domain data when tested on a single-domain test set. The aforementioned studies have focused on cross-domain misinformation detection at the content level. In contrast, our study is centered on comprehending the conduct of users involved in disseminating cross-domain misinformation through a causal framework.

\subsection{User-Centric analysis of misinformation}

One of the major focuses of interest in the work related to COVID-19 misinformation was on studying the implications of COVID-19 misinformation on various aspects related to society. In one of the popular studies, \citet{ROMER2020113356} observed that the belief in conspiracy theories prospectively predicted resistance to preventive action and vaccination among individuals. It was also observed that conservative ideology and high consumption of media were positively correlated with the degree of conspiracy belief among individuals.~\citet{islam2020covid} performed a content analysis of the news articles focusing on understanding the public perception of COVID-19-related misinformation. The authors identified 2,311 reports of rumors, stigma, and conspiracy theories in 25 languages from 87 countries, showing that conspiracy theories had serious implications on the individual and community, especially on public health. In a later study, \citet{verma2022examining} conducted a large-scale observational study spanning over 80 million Twitter posts spanning over 18 months. The authors demonstrated that users who shared COVID-19 misinformation experienced approximately two times an additional increase in anxiety when compared to similar users who did not share misinformation. Furthermore, their analysis revealed that women, racial minorities, and individuals with lower levels of education in the United States experienced a disproportionately higher increase in anxiety when compared to the other users. Moreover, their analysis showed that women, racial minorities, and individuals with lower levels of education exhibited a notably higher increase in anxiety when compared to other user cohorts, emphasizing the disparate impact of COVID-19-related misinformation on mental health within these populations. Cases of hate speech against specific communities surged during the pandemic due to the origin theories related to the virus. Focusing on the anti-Asian hate, \citet{10.1145/3487351.3488324} created the COVID-HATE dataset with over 206 million anti-Asian hate and counter-hate tweets. Using this dataset, the authors performed a  linguistic and network analysis of hate and counterspeech users. Upon exposure to counterspeech messages, individuals expressing hateful sentiments demonstrated a notable shift in behavior, showcasing a discernible influence that led to a reduction in the propagation of hate speech tweets.

Compared to COVID-19, user-centric analysis pertaining to \politics~and \climate~misinformation is under-studied. \citet{osmundsen2021partisan} analyzed 2,300 American Twitter users and observed that strong support for partisan polarization was an influential driver for sharing political misinformation. The study additionally unveiled that there is a prevalent inclination toward partisan news sources in the general landscape of social media users. Notably, this effect is most pronounced among supporters of the Republican political faction. In one of the popular works in \climate~misinformation, \citet{van2017inoculating} conducted two online experiments involving a cohort of 1,000 U.S. nationals and 2,167 workers from Amazon Mechanical Turk (MTurk). The primary objective of the study was to analyze the ways in which individuals evaluate and process consensus cues within a polarized information environment, specifically focusing on topics related to climate change. Later, \citet{benegal2018correcting} showed that publicizing the views of influential Republicans acknowledging scientific consensus on climate change can reduce the partisan gap.

Unlike prior studies, we examine the causal relationship between users' past and future engagement with COVID-19 and non-COVID (\politics~and \climate)~misinformation. Furthermore, we study the impact of the pandemic on altering the psychological behavior of the users.

